Generating Dialogue Agents via Automated Planning

Dialogue systems have many applications such as customer support or question answering. Typically they have been limited to shallow single turn interactions. However more advanced applications such as career coaching or planning a trip require a much more complex multi-turn dialogue. Current limitations of conversational systems have made it difficult to support applications that require personalization, customization and context dependent interactions. We tackle this challenging problem by using domain-independent AI planning to automatically create dialogue plans, customized to guide a dialogue towards achieving a given goal. The input includes a library of atomic dialogue actions, an initial state of the dialogue, and a goal. Dialogue plans are plugged into a dialogue system capable to orchestrate their execution. Use cases demonstrate the viability of the approach. Our work on dialogue planning has been integrated into a product, and it is in the process of being deployed into another.

==> sections/integrating-plans.tex <==
\section{Integrating Plans into a Dialogue System}
\label{plan-integration}

\towrite{Describe how the compiled plan corresponds to the dialogue plans described in the previous section.}

Recall that a dialogue plan obtained from a planning system is
a directed graph, with nodes representing states.
A unique transition originating from a state represents
a deterministic action, and multiple transitions from a given state
represent the branches of a non-deterministic action.
Transitions are labeled with one string each,
representing the name of the corresponding action and its list of zero or more arguments.
States are labeled with the predicates that are true in the state at hand.
In this section we discuss how such a plan can be integrated and executed
into a dialogue system.

Each action in the plan (string) needs to be mapped into an actual code to execute.
We call the code corresponding to an action a \emph{transformer}.
As such, each trajectory (dialogue trace) modelled in the dialogue plan
has a corresponding sequence of transformers to call.
As mentioned in Section~\ref{sec:abstraction}, not all information contained
in the dialogue context is necessarily part of the PDDL planning problem.
Transformers can use information from the dialogue context
(i.e., use part of the context as input, and modify part of the context).
This provides a mechanism through which transformers can consume (use as input)
the effects of transformers previously called in an execution trace.

\ab{
    Is ``transformer'' an established term? If not, how about renaming these?
}

When multiple branches originate in a given state of a plan,
the execution needs to decide what branch to choose.
A simple but effective approach is to associate a condition with each branch,
based on the differences between the labels of the resulting states of each branch.
Consider the example presented in Figure~\ref{fig-fsm}.
The state labeled {\sc has-recomms} has two outgoing branches, 
corresponding to two non-deterministic effects of an action corresponding to a user utterance.
Based on the differences between the labels of the two resulting states,
the condition associated with the leftmost branch is {\sc user-accept},
and the rightmost branch has the condition {\sc not-accepted}.
These are two complementary conditions, for the cases when the user has accepted
the recommendation, or the user has rejected it.

Conditions defined in such a way are evaluated when the execution trace
reaches the parent state of the corresponding branches.
The evaluation is based on context information.
More specifically, each PDDL predicate used in a condition has associated an evaluation
formula based on variables from the context.
In our running example, the predicates {\sc user-accept} and
{\sc not-accepted} are evaluated based on 
the classification (intent) of the most recent utterance
(acceptance or rejection).

A deeper discussion on monitoring the execution of a plan is beyond the scope of this paper.

\begin{comment}
%\subsection{Transformers}
\subsection{Compiling Plans into Dialogues}
\label{sec:pc}

%\cm{This an advanced feature? I'm not quite sure what it refers to.}

Dialogues can be conceived as a combination of a small set of functions \emph{transforming} the dialogue context described in Sect.~\ref{sec:abstraction}. Such dialogue transformers perform basic tasks such as saying something to the user, or asking a question. In addition, the transformer library provides composite transformers that allow to model complex dialogues in a declarative, compositional way. 

One crucial composite transformer is the finite state machine, allowing to model arbitrary dialogue plans. For example, Figure \ref{fig:transformers} depicts the translation to dialogue transformers of the plan shown in Figure \ref{fig-fsm}.

\newcommand\jcomm[1]{\textcolor[rgb]{0.18,0.49,0.19}{\textit{#1}}}
\newcommand\jstr[1]{\textcolor[rgb]{0.05,0.27,0.63}{#1}}
\begin{figure}
      \begin{footnotesize}
    \begin{Verbatim}[commandchars=\\\{\}]
\jcomm{// Initial state}
initial(\jstr{"get-recomms"}).call(seq(
    this::getRecomms,
    say(this::stringifyRecomms)
)).jumpTo(\jstr{"query-acceptance"}).always()

\jcomm{// Query user acceptance}
on(\jstr{"query-acceptance"}).call(
    clarify(\jstr{"acceptance"})
        .asking(\jstr{"Accept recommendations?"})
        .withExtractor(yesNo())
).finish().when(getBool(\jstr{"acceptance"}))
 .jumpTo(\jstr{"elicit-reject-reason"}).otherwise()

\jcomm{// Elicit reject reason}
on(\jstr{"elicit-reject-reason"}).call(
    clarify(\jstr{"reason"})
        .asking(\jstr{"Why not?"})
        .withExtractor(fromInput())
).jumpTo(\jstr{"get-recomms"}).always()
    \end{Verbatim}
\end{footnotesize}
\caption{Plan in Figure \ref{fig-fsm}, as dialogue transformers.}
\label{fig:transformers}
\end{figure}

From the initial state we call the high-level transformer \texttt{seq} to assemble the two-step sequence [\texttt{getRecomms}, \texttt{say(stringifyRecomms)}], thus retrieving recommendations and showing them to the user (using the \textit{say} transformer). This sequence represents the mapping from the \texttt{get-recomms} action in the plan to actual dialogue code. The rest of the translation is self-explanatory: the dialogue jumps unconditionally to the \texttt{query-acceptance} state, thus querying the user. Depending on the intent associated to the answer's utterance (extracted by means of a \texttt{yesNo} NLU extractor) the dialogue will finalize or go the \texttt{elicit-reject-reason} state, asking about the rejection reason. From there the dialogue will jump unconditionally to the initial state.

Since plans can be arbitrarily complex, the translation process must be automated. To this end we implemented a compiler that traverses a plan in a depth first fashion, generating the corresponding transformer ensemble along the way. The compiler requires a mapping from plan actions to transformers (e.g., \texttt{get-recomms} to the sequence [\texttt{getRecomms}, \texttt{say(stringifyRecomms)}]), and another from plan predicates to code (e.g., \texttt{user-accepted} to \texttt{getBool("acceptance")}). The ability to compile plans leverages dynamic scenarios where a planning service is invoked on the fly, and the resulting plan compiled into a dialogue and executed at runtime.

\end{comment}

